Content Filtering with Inattentive Information Consumers

We develop a model of content filtering as a game between the filter and the content consumer, where the latter incurs information costs for examining the content. Motivating examples include censoring misinformation, spam/phish filtering, and recommender systems. When the attacker is exogenous, we show that improving the filter's quality is weakly Pareto improving, but has no impact on equilibrium payoffs until the filter becomes sufficiently accurate. Further, if the filter does not internalize the information costs, its lack of commitment power may render it useless and lead to inefficient outcomes. When the attacker is also strategic, improvements to filter quality may sometimes decrease equilibrium payoffs.

==> generalization-stronger.tex <==
\section{Generalized information costs}
\label{sec:gen}

This appendix begins to generalize our notion of information costs.
Specifically, we consider convex/concave information costs (defined below). \asedit{We focus on aligned utilities, and we restrict the filter to only use pure action strategies.} We show that in some parameter regime, the differentiating profile $\difprof$ is socially optimal, and the players' utility under this profile is strictly increasing in the filter quality. \asedit{Moreover, the parameter regime(s) when this does \emph{not} happen are  essentially trivial: either the filter does not choose the differentiating strategy $\strdif$ (and players' payoffs do not depend on the filter quality), or the consumer does not incur information costs.}


%\footnote{We limit our attention to the case where the filer chooses the differentiating strategy $\strdif$, because if the filter forwards all content or blocks all content, then players' payoffs do not depend on the filter quality.}

%$\pi_0$, $-\pi_1$

Let us formulate our cost model. Let $C(\mu; q(\difprof))$ be the consumer's cost for choosing information strategy
    $\mu=\rbr{\tilde{\pi}_0, \tilde{\pi}_1}$
  when their prior belief that content is
  malicious is $q(\mixstrfil)$. We assume the following:
\begin{enumerate}
\item  $C$ is strictly convex in $\mu$;
\item $C$ is strictly concave in $q(\mixstrfil)$;
\item $ C$ is differentiable in $\mu$ and $q(\mixstrfil)$;
\item $C(\mu;q(\mixstrfil))=0$ if and only if
      $P(X|\Psi_{\texttt{c}})=P(X)$.
\end{enumerate}

\noindent Assumptions 1-3 are standard.  Assumption $4$ says that the
consumer can costlessly choose to gather no information and any
other information that shifts the distribution away from the prior must be costly.

\asedit{The main result of this section is stated as follows.}

\begin{prop}\label{prop:gen-costs}
\asedit{Consider information costs that satisfy assumptions 1-4 above. Posit aligned utilities. Restrict the filter to only use pure action strategies.}

Then there exists a parameter regime for which the differentiating profile $\difprof$ is socially optimal and
\begin{align}\label{eq:prop:gen-costs}
 \frac{\partial V(\difprof)}{\partial \pi_1}>0 \text{    and    } \frac{\partial V(\difprof)}{\partial \pi_2}<0.
\end{align}
This happens for sufficiently high costs $c_1, c_2$ and sufficiently high filter quality, namely when
    $\min(c_1,c_2)>\underline{c}$
and
    $\min(\pi_1, 1-\pi_2)>\underline{\pi}$
for some thresholds $\underline{c}>0$ and $\underline{\pi}<1$.
\end{prop}

The key reason is the following:

\begin{proposition}\label{prop:gen-costs-2}
\asedit{Make the assumptions in Proposition~\ref{prop:gen-costs}. Further, assume the parameters are such that in an open neighborhood around $(\pi_0,\pi_1)$ (and fixing the other parameters) $\difprof$ is socially optimal and the consumer incurs positive information costs under $\difprof$. Then
\refeq{eq:prop:gen-costs} holds.}
\end{proposition}

\asedit{We prove these two propositions in what follows. Throughout, we make the assumptions in Proposition~\ref{prop:gen-costs} without further notice.}

Let us adopt the following notation:
\begin{align}
\vec{q}(\mixstrfil)
    &= [q(\mixstrfil), (1-q(\mixstrfil))]^{\prime}\nonumber \\
\tilde{\Pi}(\mu)
    &= \begin{bmatrix}
        \tilde{\pi}_1 & 1-\tilde{\pi}_1 \\
        \tilde{\pi}_2 & 1-\tilde{\pi}_2
    \end{bmatrix} \nonumber \\
\vec{R}
    &= \begin{bmatrix}
            0 & -c_1 \\
            c_2 & b
    \end{bmatrix}
    \label{eq:GenCosts-notation}
\end{align}

%\ascomment{point \#1}
Under strategy profile $\difprof$, the consumer chooses information strategy
  $\mu=\rbr{\tilde{\pi}_0, \tilde{\pi}_1}$
%$\tilde{\pi}_1$ and $ \tilde{\pi}_2$
and pure action strategy $s_{\texttt{c}}$ in order to optimize
\begin{equation*}
  V_g(\difprof, s_{\texttt{c}}, \mu)
  =  \mathrm{tr}\left(\tilde{\Pi}(\mu)\vec{R}\right) \cdot \vec{q}(\difprof) - C(\mu; q(\mixstrfil)).
\end{equation*}

%\ascomment{point \#2}
The consumer has a unique optimal choice of $\mu$. This is because the consumer's strategy space is compact and $V_g$ is a concave function minus a convex function.
 \ascomment{Your point here is that this is the case for any filter's strategy, or just for $\difprof$?}

%\ascomment{point \#3}
\begin{claim}
The consumer incurs positive information costs \asedit{under $\difprof$} \ascomment{this is only about $\difprof$, right?} for sufficiently high values of $c_1$ and $c_2$.
\end{claim}
\begin{proof}
Focus on the differentiating profile $\difprof$.
The consumer incurs positive information costs
if and only if there exists an information strategy $\mu^{\prime}$ such that
$C(\mu^{\prime}, q(\difprof))>0$ and
$V_g((\mixstrfil, s_{\texttt{c}}, \mu^{\prime}))$ is strictly larger than
\[\max(-(1-q(\difprof))c_1, -q(\difprof)c_2 + (1-q(\difprof)b)). \]  
For sufficiently high values of $c_1$ and $c_2$, such a $\mu^{\prime}$ is
guaranteed to exist.
\end{proof}

%The consumer incurs positive information costs if
%and only if there exists a $\mu^{\prime}$ such that
%$C(\mu^{\prime}, q(\difprof))>0$ and
%$V_g((\mixstrfil, s_{\texttt{c}}, \mu^{\prime})) >
%\max(-(1-q(\difprof))c_1, -q(\difprof)c_2 + (1-q(\difprof)b))$.  For
%sufficiently high values of $c_1$ and $c_2$, such a $\mu^{\prime}$ is
%guaranteed to exist.

%\ascomment{point \#4}
\begin{claim}
The filter's optimal strategy is $\difprof$ for sufficiently high filter quality, specifically when $\min(\pi_1, 1-\pi_2)$ exceeds some threshold $\underline{\pi}<1$.
\end{claim}

\asedit{Now, Proposition~\ref{prop:gen-costs} follows from Proposition~\ref{prop:gen-costs-2}. It remains to prove the latter.}

\begin{proof}[Proof of Proposition~\ref{prop:gen-costs-2}]
\ascomment{so, pls fill this in. Copy and paste, hopefully.}
\end{proof}



\ascomment{OLD STUFF BELOW}

\begin{prop}
  Assume there exists a $\mu^{\prime}$ such that $V_g((\bar{s}_{\texttt{f}}, s_{\texttt{c}},
\mu^{\prime})) > \max(-(1-q(\difprof))c_1, -q(\difprof)c_2 +
(1-q(\difprof)b))$ and the socially optimal strategy for the filter is
to play a differentiating strategy.
Then:
\begin{align*}
 \frac{\partial V(\sigma^*)}{\partial \pi_1}>0 \text{    and    } \frac{\partial V(\sigma^*)}{\partial \pi_2}<0
\end{align*}
\end{prop}

\begin{proof}
  We prove the first case, the second case follows similarly
  %\begin{align*}
    %&\frac{\partial}{\partial \pi_1} \left((1-\pi_1)q + (1-\pi_2)(1-q)\right) \times \nonumber \\
    %&\left( (1-\tilde{\pi}_1)q(\difprof)-c_2 + (1-q(\difprof))(\tilde{\pi}_2-c_1 + (1-q(\difprof))(1-\tilde{\pi}_2)b - C(\mu; q(\difprof))\right)>0 \nonumber
  %\end{align*}
  %This amounts to
  \begin{align*}
    & \frac{\partial V(\sigma^*)}{\partial \pi_1} =  \nonumber \\
    & A\bigg(\left(\frac{\partial Z}{\partial \tilde{\pi}_1} +
    \frac{\partial Z}{\partial \tilde{\pi}_2}\right) \times
  \left(\frac{\partial \tilde{\pi}_1}{\partial q(\difprof)} \frac{\partial q(\difprof)}{\partial \pi_1}\right) + \nonumber \\
  & \frac{\partial Z}{\partial q(\difprof)}\frac{\partial q(\difprof)}{\partial\pi_1}\bigg) + Zq
%\label{eq:inc}
  \end{align*}
  where
  \begin{align*}
  A &= \left((1-\pi_1)q + (1-\pi_2)(1-q)\right) \\
   Z &=(
    (1-\tilde{\pi}_1)q(\difprof)(-c_2) + \\
    &(1-q(\difprof))(\tilde{\pi}_2(-c_1) +
    (1-q(\difprof))(1-\tilde{\pi}_2)b + \\
    & C(\mu; q(\difprof)))
    \end{align*}
  However, by enforcing optimality for the consumer $\frac{\partial Z}{\partial \tilde{\pi}_1}=
  \frac{\partial Z}{\partial \tilde{\pi}_2}=0$.  Therefore, it is now sufficient to show that
  \begin{align}
    (1-\tilde{\pi}_1)c_2 + (1-q(\difprof))\frac{\partial C}{\partial q(\difprof)} + C(\mu;q(\difprof))>0
    \label{eq:fin}
  \end{align}
  By the definition of concavity (and notationally dropping the
  dependence on $\mu$), it must be that
  \begin{align*}
  C(q(\difprof)') - C(q(\difprof)) < \frac{\partial{C}}{\partial q(\difprof)}(q(\difprof)' - q(\difprof))
\end{align*}
for any $q(\difprof)$ and $q(\difprof)^{\prime}$. Plugging in $1$ for
$q(\difprof)^{\prime}$ and rearranging yields
\begin{align*}
  \frac{\partial{C}}{\partial q(\difprof)}(1 - q(\difprof)) +C(q(\difprof))>C(1)>0
  \end{align*}
which then implies that inequality \eqref{eq:fin} is satisfied since the
first term is positive and the sum of the second and third term are
positive and thus completes the proof.

\end{proof}

%\jgedit{
%\begin{prop}
%    Assume the parameters are such that in a local region around $\pi_0$, $\pi_1$, the socially optimal strategy is for the filter to play $\difprof$ and the consumer to incur strictly positive information costs.  Then:
%    \begin{align*}
% \frac{\partial V(\sigma^*)}{\partial \pi_1}>0 \text{    and    } \frac{\partial V(\sigma^*)}{\partial \pi_2}<0
%\end{align*}
%\end{prop}} 

==> misaligned_bu.tex <==
%\subsection{Consumer-Only Information Costs}

% Proposition \ref{prop:dcase0} characterizes when a differentiating
% equilibrium is the socially optimal equilibrium when the consumer and
% filter have a common interest.


% \jgcomment{Move paragraph to motivation}
% However, complete alignment might not always be the case and the
% filter and the consumer may internalize the information costs
% differently.  In a security situations such as a spam filter, firms
% may purchase filtering software based on the software's advertised
% performance metrics and thus the filter does not internalize the
% consumer's deliberation costs.  As another example, a social media
% platform that has monopoly power may incur costs when misinformation
% propagates but since there is no alternative platform for the
% consumers, the platform may not (fully) internalize the consumers'
% deliberation costs.

% Instead of fully characterizing the value of information

This section considers \emph{semi-aligned utilities}:
$\Vfil(\sigma) = u(\sigma)$.  Again, when considering total welfare,
it suffices to focus on two pure strategy profiles, the
differentiating profile $\difprof$ and the forwarding profile
$\fwdprof$, since payoffs in any mixed strategy equilibrium are
bounded by the greater of $V_i(\fwdprof)$ and $V_i(\difprof)$.  

\begin{lem}\label{prop:nomixsemi}
  For any mixed strategy \emph{equilibrium}, $\mixsigma$,
  $V_i(\mixsigma)$ is upper bounded by $\max(V_i(\difprof),
  V_i(\fwdprof)$ for $i\in\{\texttt{f}, \texttt{c}\})$.  
\end{lem}

  
\begin{prop}\label{prop:semi-eq}
The differentiating profile  $\difprof$ is an equilibrium if and only if
  $\frac{\pi_0(1-\pi_1)}{\pi_1(1-\pi_0)}>\frac{b+c_1}{c_2}\frac{1-\qL}{\qL}$.
The forwarding profile $\fwdprof$ is an equilibrium if and only if
  $\frac{\pi_0}{\pi_1}<\frac{b+c_1}{c_2}\frac{1-\qL}{\qL}$.
Therefore, either $\difprof$ or $\fwdprof$ is an equilibrium (or both). The other possible equilibria are weakly Pareto-dominated by $\difprof$ and $\fwdprof$.
\end{prop}

\noindent The equilibrium condition for $\difprof$ (resp., $\fwdprof$) has a notable shape: the left-hand side depends only filter's quality $(\pi_0,\pi_1)$, and the right-hand side depends only on the payoff parameters $(b,c_1,c_2,\infoL)$.

In a stark contrast with the previous section, \asedit{we have an inefficiency:} there may be a strategy profile which Pareto-dominates every equilibrium, but nevertheless is not an equilibrium itself.

\begin{theorem}\label{thm:semi-inefficiency}
Assume  $\qL <\qdif<\qH<q$.  Then $\difprof$ strictly Pareto-dominates $\fwdprof$ (and therefore any other equilibrium), but is not an equilibrium if the respective condition in Proposition~\ref{prop:semi-eq} fails.
% \begin{align}
%   \frac{\pi_1}{\pi_2}>\frac{(1-q)(1-\tilde{\pi}^*_2)(b+c_1)}{c_2(1-\tilde{\pi}^*_1)q} \nonumber
%   \end{align}
% \begin{align}
%   \frac{\pi_1}{\pi_2}>(b+c_1) \frac{e^{b/\lambda_2} (1-e^{-c_2/\lambda_2})}{e^{-c_2/\lambda_2}(e^{b/\lambda_2} - e^{-c_1/\lambda_2})} \label{eq:noinef}
    %   \end{align}
% \begin{align}
%   \frac{\pi_0 (1-\pi_1)}{\pi_1(1-\pi_0)}>\frac{b+c_1}{c_2}\frac{1-q_H}{q_H}e^{(b+c_1+c_2)/\lambda_{\texttt{c}}} \label{eq:prop2cond}
%   \end{align}
\end{theorem}

\noindent \asedit{Essentially, in this parameter regime the filter's signal cannot sufficiently discern malicious content from clean content, so the filter cannot commit to the differentiating
strategy.}


We now characterize the value of technology (VoT). \asedit{Similar to Theorem~\ref{thm:dvdp}, we find a trichotomy into constant, linear and non-linear dependence on $(\pi_0,\pi_1)$.} However, equilibrium selection is no longer trivially resolved in favor of social optimality (as players' utilities do not coincide), so we treat $\difprof$ and $\fwdprof$ separately.


\begin{theorem}\label{thm:semi-VoT}
\begin{itemize}

\item[(a)] \emthm{Constant VoT.}
Under $\fwdprof$, we have
    $\frac{\partial{V_i(\fwdprof)}}{\partial \pi_x}=0$
for any $i\in\cbr{\fil,\con}$ and $x\in\bin$.

\item[(b)] \emthm{Piecewise-linear VoT.}
Under $\difprof$, filter's marginal VoT,
    $\frac{\partial{\Vfil(\difprof)}}{\partial \pi_x}$, $x\in\bin$,
does not depend on $(\pi_0,\pi_1)$ when $\qdif>\qL$ (resp., when $\qdif<\qL$), but does depend on $\infoL$.

\item[(c)] \emthm{Non-linear VoT.}
Under $\difprof$, consumer's VoT is non-linear: \refeq{eq:thm:dvdp-nonlinear} holds with $\Vopt = \Vcon(\difprof)$.

\end{itemize}
\end{theorem}

%\ascomment{alternative props}
%\begin{prop}[constant VoT]\label{prop:semi-VoT-fwd}
%Under $\fwdprof$, we have
%    $\frac{\partial{V_i(\fwdprof)}}{\partial \pi_x}$
%for any $i\in\cbr{\fil,\con}$ and $x\in\bin$.
%\end{prop}
%\begin{prop}\label{prop:semi-VoT-diff}
%Under $\difprof$, consumer's VoT is \emthm{non-linear} in $(\pi_0,\pi_1)$: \refeq{eq:thm:dvdp-nonlinear} holds with $\Vopt = \Vcon(\difprof)$. Filter's VoT is \emthm{piecewise linear} in $(\pi_0,\pi_1)$:
%the partial derivatives
%   $\frac{\partial{\Vfil(\difprof)}}{\partial \pi_x}$, $x\in\bin$
%do not depend on $(\pi_0,\pi_1)$ as long as $\qdif>\qL$ (resp., as long as $\qdif<\qL$). However, these partial derivatives depend on $\infoL$ (when $\qdif>\qL$ and when $\qdif<\qL$).
%\end{prop}


\asedit{As in Theorem~\ref{thm:dvdp}, non-linearity of VoT arises due to strategic interactions between the filter and the consumer. Unlike Theorem~\ref{thm:dvdp}(b), strategic considerations arise even in the linear VoT regime, since in Theorem~\ref{thm:semi-VoT}(b) filter's marginal VoT depends on $\infoL$, and hence on consumer's information costs. }

% \begin{theorem}
%   \label{thm:dvdpsemi}
%   Assume $q_L <\qdif<\qH<q$.  Then $\difprof$ is an equilibrium where
%   $\frac{\partial V_i(\difprof)}{\partial \pi_0}>0$ and
%   $\frac{\partial V_i(\difprof)}{\partial \pi_1}<0$ if and only if the
%   inequality in proposition \ref{prop:existsnoinfo} is satisfied.
%   Furthermore, if proposition \ref{prop:existsnoinfo} is not satisfied, the
%   marginal value of technolgy at any equilibrium profile is $0$.
% \end{theorem}

\medskip

 \begin{figure}
   \centering
  \includegraphics[trim=1in 0in 1in 0in,clip,width=\textwidth]{./figs/prop2_1.png}
  \ascomment{TODO: change the legend, make x-axis in terms of $\qdif$}
   \caption{Inefficiency when the filter cannot commit to the differentiating strategy $\strdif$}
   \label{fig:mis1}
 \end{figure}

\asedit{The intuition from the above results is illustrated in Figure~\ref{fig:mis1}. We focus on the same parameter regime as Figure~\ref{fig:p11} (except we now have semi-aligned utilities). In particular, we vary $\qdif$ along the x-axis while keeping $\pi_1$ fixed, where $\qdif$ characterizes the quality of filter's signal. The y-axis corresponds to filter's expected payoffs $\Vfil(\cdot)$. Specifically, the blue line is  for the differentiating profile $\difprof$, the dotted line is for the forwarding profile $\fwdprof$, and the purple line is for the strategy profile when the consumer's strategy is the same as in $\difprof$, but the filter \emph{deviates} to the forwarding strategy $\strfwd$ (call it the \emph{deviating profile} $\devprof$). Let's focus on the region $\pi_0>\pi_0^L$
\ascomment{which would be $\qdif<\qH$, right?}.
When the consumer responds optimally, the filter is better off when it differentiates: 
    $\Vfil(\difprof)>\Vfil(\fwdprof)$.
For aligned utilities, $\difprof$ is in fact an equilibrium. However, for semi-aligned utilities this is no longer true. Indeed, the filter is better off deviating, $\Vfil(\devprof)>\Vfil(\difprof)$, when $\qdif$ is in some range $q^*<\qH$ (see the pink region). }

\ascomment{Figure \ref{fig:mis2} is supposed to go away}

Figure \ref{fig:mis2} shows that this incentive to deceive the
 consumer arises because deception leads the consumer to gathering
 more information than optimal and thus provides a benefit to the
 filter.  In particular, for any values of $\pi_0$ where
 $I(\sigma^t)>I(\sigma^s)$, if the filter could convince the consumer
 that it was playing a differentiating strategy, it could deceive the
 consumer to collect more information than optimal by switching from a
 differentiating strategy to forwarding all content.  Now consider a
 value of $\pi_0$ sufficiently close to $\pi_0^L$.  The filter is
 practically indifferent between sending all content to the consumer
 and a differentiating strategy, assuming that the consumer best
 responds.  However, if the consumer \emph{incorrectly} believes that
 the filter were to differentiate, but the filter instead switches to
 forwarding all content to the consumer, the consumer then over spends
 attention resource to improve the fidelity of its signal.  This
 higher fidelity signal would then make the filter better off when it
 does not differentiate and thus the filter could not commit to
 maintaining a differentiating strategy in equilibrium.


 % At $\pi_1^L$, assuming the
 % consumer best responds to the filter, the filter is indifferent
 % between playing the differentiating strategy and passing all content
 % to the consumer.  However, since at $\pi_1^L$, the green line is
 % above the red dashed line, if the filter deviates away from
 % differentiating, the filter can ``trick'' the consumer
 % into getting a higher fidelity signal, providing a benefit to the
 % filter to the detriment of the consumer.  Of course, because the
 % filter has an

 \begin{figure}
   \centering
  \includegraphics[trim=1in 0 1in 0, width=\textwidth]{./figs/prop2_2.png}
   \caption{Inefficiency when the filter cannot commit to
     differentiating and associated consumer information costs. }
   \label{fig:mis2}
 \end{figure}

 % It would be tempting to hope that the filter can escape this lack of
 % commitment by playing a mixed strategy.  However, any mixed strategy
 % for the filter induces a unique prior for the consumer and it can be
 % shown (lemma \ref{lem:eqb} in the appendix), that the filter's best
 % response for any prior belief is unique.  Therefore, the consumer
 % would never be willing to randomize in order to make the filter
 % indifferent and also randomize.  As a result, the inefficiency of the
 % pure strategy equilibrium outcome cannot be assuaged by a mixed
 % strategy equilibrium.

%  Of course, if the filter could either enter into a binding contract
%  \emph{ex-ante} with the consumer or if consumer can directly observe
%  the filter's strategy and best respond accordingly, social optimality
%  would be restored.  However, there is another mechanism that can
%  ensure the filter plays a differentiating strategy that doesn't
%  require an \emph{ex-ante} commitment from the filter.  Suppose that
%  after the game the consumer could, through some unbiased analysis,
%  determine whether the filter played a differentiating strategy or
%  simply forwarded all content to the consumer.  Furthermore, the
%  consumer could also commit to paying the filter a fixed amount if it
%  was revealed that the filter did indeed play a differentiating
%  strategy.  The following proposition shows that there is an
%  equilibrium in which the consumer pays the filter and the filter
%  endogenously commits to a differentiating strategy as long as the
%  filter saves the consumer sufficient information costs.

% % \begin{prop}\label{prop:trans}
% %   Assume
% %   \begin{enumerate}
% %   \item $q_L <\tilde{q}<q_H$
% %   \item $\bar{V}_i >V^{\prime}$ (as in proposition \ref{prop:existsnoinfo})
% %   \item $\lambda_1=0$
% %   \item $\frac{\pi_1
% %       (1-\pi_2)}{\pi_2(1-\pi_1)}<\frac{b+c_1}{c_2}\frac{1-q_H}{q_H}e^{(b+c_1+c_2)/\lambda_2}$
% %   \end{enumerate}
% %   and let $\lambda_2\bar{I}$ and $\lambda_2I^{\prime}$ be the
% %   consumer's optimal information costs when the filter differentiates
% %   and passes all content, respectively.  Finally, let
% %   $V^{\prime \prime}$ be the filter's payoff when it always passes
% %   content but the consumer best responds as if $s_1=\bar{s}_1$.
% %   Assume that before play, both the filter that consumer can enter
% %   into a  contract where the consumer agrees to transfer
% %   utility to the filter if the filter chooses $\bar{s}_1$.  Such a
% %   contract is supported in equilibrium if and only if
% %   \begin{align}
% %     \lambda_2\left[I^{\prime} - \beta \bar{I}\right] > V^{\prime} + V^{\prime \prime} - \bar{V}
% %   \end{align}
% % \end{prop}

%  \begin{prop}
%    \label{prop:trans}
%    Under the same assumptions of proposition  \ref{prop:existsnoinfo},
%    assume the inequality in \ref{eq:prop2cond} is satisfied.  Assume
%    that before play, both the filter that consumer can enter into a
%    binding contract where the consumer agrees to transfer utility to
%    the filter if the filter chooses $\bar{s}_{\texttt{f}}$.  Such a contract is
%    supported in equilibrium if and only if
%    \begin{equation}
%      \lambda_{\texttt{c}}\left[I(\sigma^s) - \beta I(\bar{\sigma})\right] > \left(R(\sigma^t)- R(\bar{\sigma})\right) + \left(R(\sigma^s) - R(\bar{\sigma})\right)
%     \end{equation}
%  \end{prop}


%  In practical terms, proposition \ref{prop:trans} says that the
% consumer would be willing to pay the filter to commit to a
% differentiating strategy as long as the differentiating strategy
% provided the filter with a sufficient reduction in information costs.
% This elucidates the fact that consumers do not only receive a benefit
% from a reduction in exposure from malicious content but also due to a
% reduction in their deliberation costs.  Furthermore, the consumer
% would be willing to \emph{pay} for that reduction in deliberation
% costs, even if the outcomes are relatively unchanged.


% \begin{figure}
%    \centering
%   \includegraphics[trim=1in 0 1in 0, width=\textwidth]{./figs/prop3_1.png}
%    \caption{Inefficiency when the filter cannot commit to
%      differentiating but can enter a contract with the consumer.}
%    \label{fig:mis3}
%  \end{figure}

% Figure \ref{fig:mis3} shows how the introduction of an ex-post
% verifiable contract can expand the region in which $\sigma^*$ is
% supported in equilibrium.  The light blue region represents the values
% of $\pi_0$ for which without transferable utility, the only
% equilibrium was socially sub-optimal but with transfer payments restore
% social optimality.  At $\pi_0=\pi_0^{\prime}$ the vertical red line
% and the vertical blue line are exactly the same height which
% demonstrates that the amount the consumer would be willing to pay to
% switch from a sub-optimal outcome to an optimal equilibrium is exactly
% the amount the filter would have to be paid to commit to playing a
% differentiating strategy.






% % the next salient question to address
% % is the value of information when the payoffs to the user and the
% % detector are not aligned.  While there are many ways the preferences
% % for the user and the detector can differ, we focus on the case where
% % the detector does not internalize the user's information cost.
% % This
% %might be the case when a platform has a monopoloy over certain
% %content or the decision maker that purchases the product does not
% %perceive the cost of attention (a worker loses productivity but the
% %person buying the product only looks at the FP/FN rate

% % we focus on the degree to
% % which the detector internalizes the users attention costs.
% % Specifically, we introduce two new parameters $\lambda_u$ and
% % $\lambda_d$, which represents the relative importance of attention
% % costs for the user and detector, respectively.

% Figure \ref{fig:mis1} shows the user's and detector's expected payoff
% for different detector strategies when the user best responds to those
% strategies. % The attention parameter for
% % the user is the same as in figure \ref{fig:p11} but the attention
% % parameter for the detector is $0$.
% Again, in this case the detector does not internalize any of the
% user's attention costs.  The main difference in this figure is the
% change in the location in which differentiating can be optimal and the
% inefficiencies that arise.

% % \begin{figure}
% %   \centering
% % %  \includegraphics[width=.7\textwidth]{misalign1.png}
% %   \caption{$\lambda_u=2, \lambda_d=0$}
% %   \label{fig:mis1}
% % \end{figure}

% Specifically, if the detector internalized all of the user's
% information costs, differentiating could only be the detector-optimal
% equilibrium strategy for values of $\pi_1>\pi_1^{\prime}$ (where the
% solid and dotted orange lines intersect).  However, when the detector
% doesn't internalize information costs, differentiating can only be the
% detector-optimal strategy at values of $\pi_1>\pi_1^L$.

% Finally, the misalignment of payoffs introduces an inefficiency for
% some values of $\pi_1$.  Consider the point directly at $\pi_1^L$.  At
% that value, the detector is indifferent between the equilibrium in
% which it differentiates and the equilibrium in which it doesn't.
% However, the \emph{user} is better off when the detector
% differentiates.  That means if the detector were to change its
% strategy from not differentiating to differentiating there would be a
% Pareto improvement in payoffs.  It is easy to see that if we allow
% utility transfers around $\pi_1^L$, there may  be Pareto improvements
% where the detector and the user are both better off.

% Of course, this type of reasoning \emph{assumes} the detector has no
% incentive to trick the user.  That is, given the user best responds
% \emph{as if} the detector differentiates, the detector does not have
% an incentive to not differentiate.  This is yet to be proven.  To
% prove this, we have to define what it means to ``hold the user's
% utility strategy constant.''  Here we adopt the notion that the user
% holds $\tilde{\psi_1}$ and $\tilde{\psi_2}$ constant.  This implies
% that when the detector is considering deviations, it assumes the user
% still commits to the same attention strategy but because the user's
% prior is no longer correct when the detector deviates, the user's
% beliefs and information costs are not as it would have expected.


% As the next proposition shows, when the detector does not internalize
% the information costs, it lacks the commitment power to choose the
% strategy of a differentiating equilibrium and thus leads to an
% inefficiency.  However, before proving the proposition we introduct
% some slight change in notation.  Since the incentives are no longer
% aligned, let $V^*_d$ and $V^*_u$ denote the detector's and user's
% expected utility under a user-optimal differentiating profile, respectively.
% Similarly let $\hat{V}_d$ and $\hat{V}_u$ be the detector's and user's
% expected utility when the detector never blocks
% ($s_d(\phi)=\textbf{r} \forall \phi$) and the user responds
% optimally.

% \begin{prop}
%   \label{prop:existsnoinfo}
%   Assume
%   \begin{enumerate}
%     \item $\frac{e^{(b-c_2)/\lambda}- e^{-(c_1+c_2)/\lambda}}{e^{b/\lambda}-
%     e^{-(c_1+c_2)/\lambda}}  <\tilde{q}<\frac{e^{b/\lambda}
%     -e^{-c_1/\lambda}}{e^{b/\lambda}-e^{-(c_1+c_2)/\lambda}}$
% \item $V^*_d>\hat{V}_d$
% \end{enumerate}
% then $\sigma^*$ exists if and only if
% \begin{align}
%   \frac{\pi_1}{\pi_2}>\frac{(1-q)(1-\tilde{\pi}^*_2)(b+c_1)}{c_2(1-\tilde{\pi}^*_1)q} \nonumber
%   \end{align}
%   or in terms of the exogenous variables only:
% \begin{align}
%   \frac{\pi_1}{\pi_2}>(b+c_1) \frac{e^{b/\lambda} (1-e^{-c_2/\lambda})}{e^{-c_2/\lambda}(e^{b/\lambda} - e^{-c_1/\lambda})} \label{eq:noinef}
%   \end{align}
% where $\tilde{\pi}^*_1$ and $\tilde{\pi}^*_2$ are the user's optimal signal
% under $\sigma^*$.
% \end{prop}

% Proposition \ref{prop:existsnoinfo} says that even if the detector
% prefers the outcome when it differentiates and the user responds
% optimally to the outcome when it doesn't differentiate and the user
% responds optimally, differentiating can only be an equilibrium if a
% certain condition is met.  The following corollary shows that there
% are parameter regimes that satisfy the conditions in
% \ref{prop:existsnoinfo} but that assumptions $1$ and $2$ are not
% sufficient for $\sigma^*$ to exists.

% \begin{cor}
%   Set $q=.5$ and $c_1=0$, then for sufficiently low $\pi_1$,$\pi_2$ and $\lambda$
%   \begin{enumerate}
%     \item for sufficiently high values of $b$, assumptions $1$ and $2$
%       of proposition and inequality \ref{eq:noinf} are satisfied.
%     \item for sufficiently low values of $b$, assumptions $1$ and $2$
%       are satisfied but inequality \ref{eq:noinf} is not satisfied.
%     \end{enumerate}
%   \end{cor}




% \begin{figure}
%   \centering
% %  \includegraphics[width=.7\textwidth]{deviate1.png}
%   \caption{$\lambda_u=2, \lambda_d=0$}
%   \label{fig:mis1}
% \end{figure}


==> misaligned_jg_edits.tex <==
%\subsection{Consumer-Only Information Costs}

% Proposition \ref{prop:dcase0} characterizes when a differentiating
% equilibrium is the socially optimal equilibrium when the consumer and
% filter have a common interest.


% \jgcomment{Move paragraph to motivation}
% However, complete alignment might not always be the case and the
% filter and the consumer may internalize the information costs
% differently.  In a security situations such as a spam filter, firms
% may purchase filtering software based on the software's advertised
% performance metrics and thus the filter does not internalize the
% consumer's deliberation costs.  As another example, a social media
% platform that has monopoly power may incur costs when misinformation
% propagates but since there is no alternative platform for the
% consumers, the platform may not (fully) internalize the consumers'
% deliberation costs.

% Instead of fully characterizing the value of information

This section considers \emph{semi-aligned utilities}:
    $\Vfil(\sigma) = u(\sigma)$.
In a stark contrast with the previous section, we have an inefficiency: there may be a strategy profile which Pareto-dominates every equilibrium, but nevertheless is not an equilibrium itself.

\begin{theorem}\label{thm:semi-inefficiency}
Assume  $\qL <\qdif<\qH<q$.  Then $\difprof$ strictly Pareto-dominates any equilibrium, but is not an equilibrium itself in some parameter regime (spelled out in Proposition~\ref{prop:semi-eq}).
\end{theorem}

\noindent Essentially, in this parameter regime the filter's signal cannot sufficiently discern malicious content from clean content, so the filter cannot commit to the differentiating
strategy.

Next, we characterize equilibrium selection. \jgcomment{I'm pretty
  sure we don't want to say we characterize equilibrium
  ``selection''.  We characterize the existence of equilibria and then
  maybe talk about the existence of a Pareto dominant profile (in some
  case) among the equilibria, but we are not saying anything about
  selection when there are multiple.} It is more complicated
compared to the case of aligned utilities (where it is essentially
resolved by Proposition~\ref{prop:aligned-best-eq}). While we focus on
$\difprof$ and $\fwdprof$ as before, these two profiles are
Pareto-incomparable for some parameter regimes, \ie one may be better
for the filter, and another for the consumer. Moreover, there may be a
mixed strategy profile which is Pareto-incomparable with one or both
of them.  

Nevertheless, we identify some order.  

%Again, when considering total welfare, it suffices to

%since payoffs in any mixed strategy equilibrium are bounded by the greater of $V_i(\fwdprof)$ and $V_i(\difprof)$.

\begin{lem}\label{prop:nomixsemi}
\asedit{$V_i(\mixsigma)\leq \max\rbr{V_i(\difprof), V_i(\fwdprof)}$
for $i\in\{\texttt{f}, \texttt{c}\}$ and any mixed equilibrium $\mixsigma$.}
% For any mixed strategy \emph{equilibrium}, $\mixsigma$,
%  $V_i(\mixsigma)$ is upper bounded by $\max(V_i(\difprof),
%  V_i(\fwdprof)$ for $i\in\{\texttt{f}, \texttt{c}\}$.
\end{lem}

\begin{prop}\label{prop:semi-eq}
The differentiating profile  $\difprof$ is an equilibrium iff
  $\frac{\pi_0(1-\pi_1)}{\pi_1(1-\pi_0)}>\frac{b+c_1}{c_2}\frac{1-\qL}{\qL}$.
The forwarding profile $\fwdprof$ is an equilibrium iff
  $\frac{\pi_0}{\pi_1}<\frac{b+c_1}{c_2}\frac{1-\qL}{\qL}$.  A mixed
  strategy equilibrium exists if and only if both $\fwdprof$ and
  $\difprof$ exists as an equilibrium.
\jgdelete{So, either $\difprof$ or $\fwdprof$ is an equilibrium (or both).}
\asdelete{The other possible equilibria are weakly Pareto-dominated by $\difprof$ or $\fwdprof$.}
\end{prop}

\noindent The equilibrium condition for $\difprof$ (resp., $\fwdprof$) has a notable shape: the left-hand side depends only filter's quality $(\pi_0,\pi_1)$, and the right-hand side depends only on the payoff parameters $(b,c_1,c_2,\infoL)$.



\begin{rem}\label{rem:semi-complicated}
Equilibrium selection is no longer trivially resolved by Proposition~\ref{prop:aligned-best-eq}. Instead, the situation is more complicated: $\fwdprof$ and $\difprof$ are Pareto-incomparable for some parameter regimes (\ie one may be better for the filter, and another for the consumer). Moreover, there may be a mixed strategy profile which is Pareto-incomparable with one or both of them.
\end{rem}

We now characterize the value of technology (VoT) for $\fwdprof$ and $\difprof$. \asedit{Similar to Theorem~\ref{thm:dvdp}, we find a trichotomy into constant, linear and non-linear dependence on $(\pi_0,\pi_1)$.}
However, we treat $\difprof$ and $\fwdprof$ separately, in view of Remark~\ref{rem:semi-complicated}. %\asedit{since equilibrium selection is no longer trivially resolved by Proposition~\ref{prop:aligned-best-eq}.}



\begin{theorem}\label{thm:semi-VoT}
\begin{itemize}

\item[(a)] \emthm{Constant VoT.}
Under $\fwdprof$, we have
    $\frac{\partial{V_i(\fwdprof)}}{\partial \pi_x}=0$
for any $i\in\cbr{\fil,\con}$ and $x\in\bin$.

\item[(b)] \emthm{Piecewise-linear VoT.}
Under $\difprof$, filter's marginal VoT,
    $\frac{\partial{\Vfil(\difprof)}}{\partial \pi_x}$, $x\in\bin$,
does not depend on $(\pi_0,\pi_1)$ when $\qdif>\qL$ (resp., when $\qdif<\qL$), but does depend on $\infoL$.

\item[(c)] \emthm{Non-linear VoT.}
Under $\difprof$, consumer's VoT is non-linear:
\refeq{eq:thm:dvdp-nonlinear} holds with $\Vopt = \Vcon(\difprof)$.

\item[(d)] \emthm{VoT at Mixed Equilibrium}
  Under the mixed equilibrium VoT for the filter is linear and
  positive and is negative and non-linear for the consumer.  

\end{itemize}
\end{theorem}

%\ascomment{alternative props}
%\begin{prop}[constant VoT]\label{prop:semi-VoT-fwd}
%Under $\fwdprof$, we have
%    $\frac{\partial{V_i(\fwdprof)}}{\partial \pi_x}$
%for any $i\in\cbr{\fil,\con}$ and $x\in\bin$.
%\end{prop}
%\begin{prop}\label{prop:semi-VoT-diff}
%Under $\difprof$, consumer's VoT is \emthm{non-linear} in $(\pi_0,\pi_1)$: \refeq{eq:thm:dvdp-nonlinear} holds with $\Vopt = \Vcon(\difprof)$. Filter's VoT is \emthm{piecewise linear} in $(\pi_0,\pi_1)$:
%the partial derivatives
%   $\frac{\partial{\Vfil(\difprof)}}{\partial \pi_x}$, $x\in\bin$
%do not depend on $(\pi_0,\pi_1)$ as long as $\qdif>\qL$ (resp., as long as $\qdif<\qL$). However, these partial derivatives depend on $\infoL$ (when $\qdif>\qL$ and when $\qdif<\qL$).
%\end{prop}


\asedit{As in Theorem~\ref{thm:dvdp}, non-linearity of VoT arises due to strategic interactions between the filter and the consumer. Unlike Theorem~\ref{thm:dvdp}(b), strategic considerations arise even in the linear VoT regime, since in Theorem~\ref{thm:semi-VoT}(b) filter's marginal VoT depends on $\infoL$, and hence on consumer's information costs. }

% \begin{theorem}
%   \label{thm:dvdpsemi}
%   Assume $q_L <\qdif<\qH<q$.  Then $\difprof$ is an equilibrium where
%   $\frac{\partial V_i(\difprof)}{\partial \pi_0}>0$ and
%   $\frac{\partial V_i(\difprof)}{\partial \pi_1}<0$ if and only if the
%   inequality in proposition \ref{prop:existsnoinfo} is satisfied.
%   Furthermore, if proposition \ref{prop:existsnoinfo} is not satisfied, the
%   marginal value of technolgy at any equilibrium profile is $0$.
% \end{theorem}

\medskip

 \begin{figure}
   \centering
  \includegraphics[trim=1in 0in 1in 0in,clip,width=\textwidth]{./figs/prop2_1.png}
  \ascomment{TODO: change the legend, make x-axis in terms of $\qdif$}
   \caption{Inefficiency when the filter cannot commit to the differentiating strategy $\strdif$}
   \label{fig:mis1}
 \end{figure}

\asedit{The intuition from the above results is illustrated in Figure~\ref{fig:mis1}. We focus on the same parameter regime as Figure~\ref{fig:p11} (except we now have semi-aligned utilities). In particular, we vary $\qdif$ along the x-axis while keeping $\pi_1$ fixed, where $\qdif$ characterizes the quality of filter's signal. The y-axis corresponds to filter's expected payoffs $\Vfil(\cdot)$. Specifically, the blue line is  for the differentiating profile $\difprof$, the dotted line is for the forwarding profile $\fwdprof$, and the purple line is for the strategy profile when the consumer's strategy is the same as in $\difprof$, but the filter \emph{deviates} to the forwarding strategy $\strfwd$ (call it the \emph{deviating profile} $\devprof$). Let's focus on the region $\pi_0>\pi_0^L$
\ascomment{which would be $\qdif<\qH$, right?}.
When the consumer responds optimally, the filter is better off when it differentiates:
    $\Vfil(\difprof)>\Vfil(\fwdprof)$.
For aligned utilities, $\difprof$ is in fact an equilibrium. However, for semi-aligned utilities this is no longer true. Indeed, the filter is better off deviating, $\Vfil(\devprof)>\Vfil(\difprof)$, when $\qdif$ is in some range $q^*<\qH$ (see the pink region). }

\ascomment{Figure \ref{fig:mis2} is supposed to go away}

Figure \ref{fig:mis2} shows that this incentive to deceive the
 consumer arises because deception leads the consumer to gathering
 more information than optimal and thus provides a benefit to the
 filter.  In particular, for any values of $\pi_0$ where
 $I(\sigma^t)>I(\sigma^s)$, if the filter could convince the consumer
 that it was playing a differentiating strategy, it could deceive the
 consumer to collect more information than optimal by switching from a
 differentiating strategy to forwarding all content.  Now consider a
 value of $\pi_0$ sufficiently close to $\pi_0^L$.  The filter is
 practically indifferent between sending all content to the consumer
 and a differentiating strategy, assuming that the consumer best
 responds.  However, if the consumer \emph{incorrectly} believes that
 the filter were to differentiate, but the filter instead switches to
 forwarding all content to the consumer, the consumer then over spends
 attention resource to improve the fidelity of its signal.  This
 higher fidelity signal would then make the filter better off when it
 does not differentiate and thus the filter could not commit to
 maintaining a differentiating strategy in equilibrium.


 % At $\pi_1^L$, assuming the
 % consumer best responds to the filter, the filter is indifferent
 % between playing the differentiating strategy and passing all content
 % to the consumer.  However, since at $\pi_1^L$, the green line is
 % above the red dashed line, if the filter deviates away from
 % differentiating, the filter can ``trick'' the consumer
 % into getting a higher fidelity signal, providing a benefit to the
 % filter to the detriment of the consumer.  Of course, because the
 % filter has an

 \begin{figure}
   \centering
  \includegraphics[trim=1in 0 1in 0, width=\textwidth]{./figs/prop2_2.png}
   \caption{Inefficiency when the filter cannot commit to
     differentiating and associated consumer information costs. }
   \label{fig:mis2}
 \end{figure}

 % It would be tempting to hope that the filter can escape this lack of
 % commitment by playing a mixed strategy.  However, any mixed strategy
 % for the filter induces a unique prior for the consumer and it can be
 % shown (lemma \ref{lem:eqb} in the appendix), that the filter's best
 % response for any prior belief is unique.  Therefore, the consumer
 % would never be willing to randomize in order to make the filter
 % indifferent and also randomize.  As a result, the inefficiency of the
 % pure strategy equilibrium outcome cannot be assuaged by a mixed
 % strategy equilibrium.

%  Of course, if the filter could either enter into a binding contract
%  \emph{ex-ante} with the consumer or if consumer can directly observe
%  the filter's strategy and best respond accordingly, social optimality
%  would be restored.  However, there is another mechanism that can
%  ensure the filter plays a differentiating strategy that doesn't
%  require an \emph{ex-ante} commitment from the filter.  Suppose that
%  after the game the consumer could, through some unbiased analysis,
%  determine whether the filter played a differentiating strategy or
%  simply forwarded all content to the consumer.  Furthermore, the
%  consumer could also commit to paying the filter a fixed amount if it
%  was revealed that the filter did indeed play a differentiating
%  strategy.  The following proposition shows that there is an
%  equilibrium in which the consumer pays the filter and the filter
%  endogenously commits to a differentiating strategy as long as the
%  filter saves the consumer sufficient information costs.

% % \begin{prop}\label{prop:trans}
% %   Assume
% %   \begin{enumerate}
% %   \item $q_L <\tilde{q}<q_H$
% %   \item $\bar{V}_i >V^{\prime}$ (as in proposition \ref{prop:existsnoinfo})
% %   \item $\lambda_1=0$
% %   \item $\frac{\pi_1
% %       (1-\pi_2)}{\pi_2(1-\pi_1)}<\frac{b+c_1}{c_2}\frac{1-q_H}{q_H}e^{(b+c_1+c_2)/\lambda_2}$
% %   \end{enumerate}
% %   and let $\lambda_2\bar{I}$ and $\lambda_2I^{\prime}$ be the
% %   consumer's optimal information costs when the filter differentiates
% %   and passes all content, respectively.  Finally, let
% %   $V^{\prime \prime}$ be the filter's payoff when it always passes
% %   content but the consumer best responds as if $s_1=\bar{s}_1$.
% %   Assume that before play, both the filter that consumer can enter
% %   into a  contract where the consumer agrees to transfer
% %   utility to the filter if the filter chooses $\bar{s}_1$.  Such a
% %   contract is supported in equilibrium if and only if
% %   \begin{align}
% %     \lambda_2\left[I^{\prime} - \beta \bar{I}\right] > V^{\prime} + V^{\prime \prime} - \bar{V}
% %   \end{align}
% % \end{prop}

%  \begin{prop}
%    \label{prop:trans}
%    Under the same assumptions of proposition  \ref{prop:existsnoinfo},
%    assume the inequality in \ref{eq:prop2cond} is satisfied.  Assume
%    that before play, both the filter that consumer can enter into a
%    binding contract where the consumer agrees to transfer utility to
%    the filter if the filter chooses $\bar{s}_{\texttt{f}}$.  Such a contract is
%    supported in equilibrium if and only if
%    \begin{equation}
%      \lambda_{\texttt{c}}\left[I(\sigma^s) - \beta I(\bar{\sigma})\right] > \left(R(\sigma^t)- R(\bar{\sigma})\right) + \left(R(\sigma^s) - R(\bar{\sigma})\right)
%     \end{equation}
%  \end{prop}


%  In practical terms, proposition \ref{prop:trans} says that the
% consumer would be willing to pay the filter to commit to a
% differentiating strategy as long as the differentiating strategy
% provided the filter with a sufficient reduction in information costs.
% This elucidates the fact that consumers do not only receive a benefit
% from a reduction in exposure from malicious content but also due to a
% reduction in their deliberation costs.  Furthermore, the consumer
% would be willing to \emph{pay} for that reduction in deliberation
% costs, even if the outcomes are relatively unchanged.


% \begin{figure}
%    \centering
%   \includegraphics[trim=1in 0 1in 0, width=\textwidth]{./figs/prop3_1.png}
%    \caption{Inefficiency when the filter cannot commit to
%      differentiating but can enter a contract with the consumer.}
%    \label{fig:mis3}
%  \end{figure}

% Figure \ref{fig:mis3} shows how the introduction of an ex-post
% verifiable contract can expand the region in which $\sigma^*$ is
% supported in equilibrium.  The light blue region represents the values
% of $\pi_0$ for which without transferable utility, the only
% equilibrium was socially sub-optimal but with transfer payments restore
% social optimality.  At $\pi_0=\pi_0^{\prime}$ the vertical red line
% and the vertical blue line are exactly the same height which
% demonstrates that the amount the consumer would be willing to pay to
% switch from a sub-optimal outcome to an optimal equilibrium is exactly
% the amount the filter would have to be paid to commit to playing a
% differentiating strategy.






% % the next salient question to address
% % is the value of information when the payoffs to the user and the
% % detector are not aligned.  While there are many ways the preferences
% % for the user and the detector can differ, we focus on the case where
% % the detector does not internalize the user's information cost.
% % This
% %might be the case when a platform has a monopoloy over certain
% %content or the decision maker that purchases the product does not
% %perceive the cost of attention (a worker loses productivity but the
% %person buying the product only looks at the FP/FN rate

% % we focus on the degree to
% % which the detector internalizes the users attention costs.
% % Specifically, we introduce two new parameters $\lambda_u$ and
% % $\lambda_d$, which represents the relative importance of attention
% % costs for the user and detector, respectively.

% Figure \ref{fig:mis1} shows the user's and detector's expected payoff
% for different detector strategies when the user best responds to those
% strategies. % The attention parameter for
% % the user is the same as in figure \ref{fig:p11} but the attention
% % parameter for the detector is $0$.
% Again, in this case the detector does not internalize any of the
% user's attention costs.  The main difference in this figure is the
% change in the location in which differentiating can be optimal and the
% inefficiencies that arise.

% % \begin{figure}
% %   \centering
% % %  \includegraphics[width=.7\textwidth]{misalign1.png}
% %   \caption{$\lambda_u=2, \lambda_d=0$}
% %   \label{fig:mis1}
% % \end{figure}

% Specifically, if the detector internalized all of the user's
% information costs, differentiating could only be the detector-optimal
% equilibrium strategy for values of $\pi_1>\pi_1^{\prime}$ (where the
% solid and dotted orange lines intersect).  However, when the detector
% doesn't internalize information costs, differentiating can only be the
% detector-optimal strategy at values of $\pi_1>\pi_1^L$.

% Finally, the misalignment of payoffs introduces an inefficiency for
% some values of $\pi_1$.  Consider the point directly at $\pi_1^L$.  At
% that value, the detector is indifferent between the equilibrium in
% which it differentiates and the equilibrium in which it doesn't.
% However, the \emph{user} is better off when the detector
% differentiates.  That means if the detector were to change its
% strategy from not differentiating to differentiating there would be a
% Pareto improvement in payoffs.  It is easy to see that if we allow
% utility transfers around $\pi_1^L$, there may  be Pareto improvements
% where the detector and the user are both better off.

% Of course, this type of reasoning \emph{assumes} the detector has no
% incentive to trick the user.  That is, given the user best responds
% \emph{as if} the detector differentiates, the detector does not have
% an incentive to not differentiate.  This is yet to be proven.  To
% prove this, we have to define what it means to ``hold the user's
% utility strategy constant.''  Here we adopt the notion that the user
% holds $\tilde{\psi_1}$ and $\tilde{\psi_2}$ constant.  This implies
% that when the detector is considering deviations, it assumes the user
% still commits to the same attention strategy but because the user's
% prior is no longer correct when the detector deviates, the user's
% beliefs and information costs are not as it would have expected.


% As the next proposition shows, when the detector does not internalize
% the information costs, it lacks the commitment power to choose the
% strategy of a differentiating equilibrium and thus leads to an
% inefficiency.  However, before proving the proposition we introduct
% some slight change in notation.  Since the incentives are no longer
% aligned, let $V^*_d$ and $V^*_u$ denote the detector's and user's
% expected utility under a user-optimal differentiating profile, respectively.
% Similarly let $\hat{V}_d$ and $\hat{V}_u$ be the detector's and user's
% expected utility when the detector never blocks
% ($s_d(\phi)=\textbf{r} \forall \phi$) and the user responds
% optimally.

% \begin{prop}
%   \label{prop:existsnoinfo}
%   Assume
%   \begin{enumerate}
%     \item $\frac{e^{(b-c_2)/\lambda}- e^{-(c_1+c_2)/\lambda}}{e^{b/\lambda}-
%     e^{-(c_1+c_2)/\lambda}}  <\tilde{q}<\frac{e^{b/\lambda}
%     -e^{-c_1/\lambda}}{e^{b/\lambda}-e^{-(c_1+c_2)/\lambda}}$
% \item $V^*_d>\hat{V}_d$
% \end{enumerate}
% then $\sigma^*$ exists if and only if
% \begin{align}
%   \frac{\pi_1}{\pi_2}>\frac{(1-q)(1-\tilde{\pi}^*_2)(b+c_1)}{c_2(1-\tilde{\pi}^*_1)q} \nonumber
%   \end{align}
%   or in terms of the exogenous variables only:
% \begin{align}
%   \frac{\pi_1}{\pi_2}>(b+c_1) \frac{e^{b/\lambda} (1-e^{-c_2/\lambda})}{e^{-c_2/\lambda}(e^{b/\lambda} - e^{-c_1/\lambda})} \label{eq:noinef}
%   \end{align}
% where $\tilde{\pi}^*_1$ and $\tilde{\pi}^*_2$ are the user's optimal signal
% under $\sigma^*$.
% \end{prop}

% Proposition \ref{prop:existsnoinfo} says that even if the detector
% prefers the outcome when it differentiates and the user responds
% optimally to the outcome when it doesn't differentiate and the user
% responds optimally, differentiating can only be an equilibrium if a
% certain condition is met.  The following corollary shows that there
% are parameter regimes that satisfy the conditions in
% \ref{prop:existsnoinfo} but that assumptions $1$ and $2$ are not
% sufficient for $\sigma^*$ to exists.

% \begin{cor}
%   Set $q=.5$ and $c_1=0$, then for sufficiently low $\pi_1$,$\pi_2$ and $\lambda$
%   \begin{enumerate}
%     \item for sufficiently high values of $b$, assumptions $1$ and $2$
%       of proposition and inequality \ref{eq:noinf} are satisfied.
%     \item for sufficiently low values of $b$, assumptions $1$ and $2$
%       are satisfied but inequality \ref{eq:noinf} is not satisfied.
%     \end{enumerate}
%   \end{cor}




% \begin{figure}
%   \centering
% %  \includegraphics[width=.7\textwidth]{deviate1.png}
%   \caption{$\lambda_u=2, \lambda_d=0$}
%   \label{fig:mis1}
% \end{figure}


==> model-Jan17.tex <==
The strategic scenario involves an information filter, denoted with
subscripts $\fil$, and an information consumer denoted with
subscripts $\con$.  In the game, the filter decides whether
to allow content to reach the consumer, and the consumer decides how
much attention to devote to determining if the content is legitimate
or malicious.  The strategic scenario unfolds in a sequence of
discrete steps.  Initially, a Bernoulli random variable $X$ with
outcomes in $\Omega_X = \{0,1\}$ determines whether the content is
legitimate or malicious with $0$ representing malicious and $1$
representing legitimate content and $q$ the prior probability that the
content is malicious.

The filter then receives a private
signal that is (possibly) correlated with the content type.  This
signal corresponds to features of the content.  For example, in the
email filtering case, the signal might represent the sender's domain or a
more sophisticated machine learning interpretation of the content's
text.  Technically, the signal $\sfil$ is a random variable with outcomes in
$\Omega_{\sfil} = \{0,1\}$.  The density of $\sfil$ conditional on $X$ is given
by $f$ where $f(0|0) = \pi_0$ and $f(0|1)=\pi_1$.  Without loss of
generality,  assume that $\pi_0\geq\pi_1$.  This means that when the
filter observes $\sfil=0$ it is more certain that the content is
malicious than if it were to observe $\sfil=1$.


%We sometimes refer to $\phi_1$ is the ``malicious
% observation'' and $\phi_2$ as the ``legitimate observation.''

After making its observation, the filter chooses to either block the
content or to pass it to the consumer.  Formally, the filter's (pure)
strategy is a function $s_{\fil}(\Phi):\{0,1\} \rightarrow \{0,1\}$, where
$0$ represents blocking and $1$ represents passing the content to the
consumer. If the filter blocks, the game ends.

If the filter passes the content to the consumer, then
the consumer updates its prior taking into account that the filter did
not block the content. The consumer then makes two decisions in
sequence.  First, it chooses how much attention to allocate to
determining the legitimacy of the content, and then it chooses to
either accept the content or ignore it.  Examples of accepting content
include believing in the veracity of a post on social media or
entering credentials into a website log-on page.  Ignoring content
represents deleting an email because it is spam or rejecting the
recommendation from a recommender system.


Formally, there is a random variable $\scon$ with outcomes in
$\Omega_{\scon} = \{0,1\}$.  Importantly, the consumer \emph{chooses}
a conditional density $g(\scon|X)$.  In principle, the signal space
can be arbitrarily large but it can be shown that any equilibrium will
only have positive weight on at most as many signals as there are
states \cite{gen1}, which in this case is two.  As shorthand, let
$\tilde{\pi}_0=g(0|0)$ and $\tilde{\pi}_1=g(0|1)$.  Since signals
determine actions, $\tilde{\pi}_0$ can be thought of as the probability
that the consumer receives a signal inducing it to ignore the content
when the content is actually malicious.  Similarly, $\tilde{\pi}_1$ is
the probability the consumer receives the signal inducing it to ignore
legitimate content.  To be clear, the consumer does not have to follow
the recommendation of the signal and will only do so in equilibrium if
it is optimal.

Let $\mu\in [0,1]^2=(\tilde{\pi}_0, \tilde{\pi}_1)$ represent the
consumer's choice of information structure or nominally the
consumer's \emph{information strategy}.  It is this choice of
information strategy that generates the consumer's information cost
through the effect it has on the consumer's posterior assessment of
whether the content is malicious or legitimate. The precise functional
form of the information cost is described in detail below.  Given its
choice of information structure, the consumer also chooses an
observation-contingent action.  Formally, the consumer's \emph{action
  strategy} is a function $s_{\con}(\scon) :\{0,1\} \rightarrow \{0,1\}$
mapping the signal to an action where $0$ represents ignoring content
and $1$ represents accepting content.

For a given realization of the game, let $a_{\fil}$ and
$a_{\con}$ be the filter's and consumer's chosen action,
respectively.  In the simple model, the only difference in the
incentives between the filter and the consumer is the degree to which
the filter internalizes the consumer's information costs.  While this
is a strong assumption, it greatly reduces the parameter space of the
model and approximates the case where the consumer and the filter's
incentive's are tightly aligned. Despite this simplifying assumption
the model is still sufficiently rich to understand the interaction
between a strategic filter and an inattentive consumer.  The payoffs
associated with the players' actions are given in table
\ref{tab:payoffs}.


\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
                   & $X=0$  & $X=1$  \\ \hline

$a_{\fil}\times a_{\con}=0$  & 0      & $-c_1$ \\ \hline

$a_{\fil} \times a_{\con}=1$ & $-c_2$ & $b$    \\ \hline
\end{tabular}
\caption{Payoffs not including information costs}
\label{tab:payoffs}
\end{table}


We call the payoffs in table \ref{tab:payoffs} the \emph{outcome
  payoffs}, and they represent the costs and benefits associated with
correct classifications and type I and type II errors.  Specifically,
if either the filter blocks or the consumer ignores malicious content,
the payoff is normalized to $0$.  If the filter blocks legitimate
content or the consumer ignores legitimate content, the payoff to both
players is $-c_1$.  If the filter fails to block malicious content and
the consumer accepts it, then the payoff is $-c_2$.  Finally, if the
consumer accepts legitimate content, the players earn a payoff of $b$.
All parameters are weakly positive.

The information cost depends on the consumer's choice of signal
distribution, the filter's strategy and other parameters of the model.
As previously mentioned, we adopt the mutual information cost function
that is common in the rational inattention literature.  Specifically,
the information cost for player $i \in \{\fil, \con\}$ is given by
\begin{align}
  \lambda_i I(X, \scon|a_{\fil}=1 ) &= \lambda_i \big[ H(X|a_{\fil} = 1) - H(\scon|X, a_{\fil}=1)\big]
                               % &= \lambda\left[ H(\omega|s_d = r) - \mathbb{E}_{\tilde{\psi}} H(\omega|\tilde{\psi}, s_d = r)\right] \nonumber \\
                               %  &= \lambda\left[ H(\tilde{\psi}|s_d=r) - \mathbb{E}_{\omega|s_d=r} H(\tilde{\psi}|\omega, s_d = r)\right] \nonumber
\label{eq:mi}
\end{align}
where $H(X)$ is the entropy of the consumer's prior, $I(X,\scon)$
is the mutual information between the consumer's prior and its choice
of signal, and $H(\scon|X)$ is the conditional entropy of the
consumer's signal.  % \bl{Is there any hope to extend, e.g., Proposition~\ref{prop:dcase0} (aligned incentives) to more general information cost functions, perhaps only requiring convexity in $\tilde{\pi}_1$ and $\tilde{\pi}_2$ and concavity in the prior, conditional on $a_1 = 1$?}
% To capture the notion that the consumer and
% filter incur information costs differently, $i$ can be either $1$ or
% $2$, representing the relative importance of information to the filter
% and consumer, respectively.

Equation \ref{eq:mi} says that the information cost is proportional to
the expected reduction in the consumer's uncertainty between its prior
and its posterior, where uncertainty of a distribution is given by its
entropy.  Equation \ref{eq:mi} also highlights the strategic
implications of the filter's choice of strategy.  Specifically, the
information costs the consumer incurs depends on its prior belief over
states of the world \emph{conditional on the filter not blocking}
($a_{\fil}=1$).  Since changes in the filter's strategy changes the
consumer's prior beliefs, the filter's choice of strategy not only
impacts the outcome payoffs but also impacts how the consumer
optimally chooses to incur information costs.

Putting the outcome payoffs and the information costs together, let
$R(X, a_{\fil}, a_{\con})$ be a function capturing the payoffs in table
\ref{tab:payoffs}.  Recalling that
$\mu=\{\tilde{\pi}_0, \tilde{\pi}_1\}$, let $\sigma = (s_{\fil}, s_{\con}, \mu)$
be a joint strategy profile.  Then the expected utility for player
$i=\fil,\con$ can be written as
\begin{equation}
  V_i(\sigma) = \mathbb{E}_{X,\sfil,\scon} \left[R\left(X,s_{\fil}(\sfil), s_{\con}(\scon)\right) -
    \mathbb{I}[s_{\fil}(\sfil)=1] \big(\lambda_i I(X, \scon | a_{\fil}=1)\big)\right] \label{eq:V}
  \end{equation}
  where the $\lambda_i$ parameter controls the relative cost of
  information for player $i$.  The consumer's choice of signal $\mu$, enters
  both directly into the information cost term as well as the
  probabilities in the expectation.  As short hand, for a strategy profile
  $\sigma$, we will write $I(X, \scon |a_{\fil}=1)$ as $I(\sigma)$ to denote
  the information costs and
  $\mathbb{E}_{X, \sfil, \scon}\left[R_i(X,s_{\fil}(\sfil),
    s_{\con}(\scon))\right]$ as $R(\sigma)$ to denote the expected
  outcome payoffs.  A Perfect Bayesian equilibrium (henceforth
  equilibrium) is then one in
  which the players choose their strategies to maximize $V_i$ under
  the usual constraints that beliefs are updated through Bayes rule.




==> old-model.tex <==
\nicomment{ah alex, using the package :)}

We consider the \emph{\ourGame}: a game between two strategic players, an information filter and an information consumer. We call them the \emph{filter} and the \emph{consumer}, and denote the respective notation with subscripts $\fil$ and $\con$. The game focuses on a single piece of content (henceforth, the \emph{content}) which can be either legitimate or malicious. The content may correspond, \eg to an email, a social media post, a recommendation, or a login prompt. The content's legitimacy is set exogenously, and is only revealed to the players via imprecise and noisy signals: via a classification algorithm (for the filter) and costly manual examination (for the consumer). Both players are incentivized to ensure that legitimate content is accepted as such, while malicious content is ignored. However, the consumer's \emph{information costs} for examining the message lead to a complex strategic interaction which we explore in this paper.

The game unfolds in several discrete steps, whereby the filter examines the content and decides whether to propagate it to the consumer, and then the consumer examines the content and decides whether to accept it as legitimate or ignore it. In detail, the protocol of the game is as follows. \nicomment{will have to justify all the binary assumptions here (e.g., classifier might give a confidence bound, gmail has a msg that is ``this looks like spam'' as well as a behavior that sends directly to spam so in essence has three, not two, msgs, etc.)}

\begin{enumerate}

\item The \emph{content type} $X\in\bin$ is realized. Formally, $X$ is a Bernoulli random variable
%with outcomes in $\Omega_X = \{0,1\}$
which determines whether the content is legitimate ($X=1$) or malicious ($X=0$). While the distribution of $X$ is known, its realization is not.
%Let $q = \Pr[X=0]$ be the prior probability that the content is malicious.

\item The filter examines the content, and receives a private signal $\sfil\in\bin$ about the content type. The signal represents the output of a classifier, so that $\sfil=0$ means ``likely malicious" and $\sfil=1$ means ``likely legitimate". The signal is drawn independently from a known conditional distribution
        $\ffil\rbr{\cdot\mid X} = \Pr\sbr{\sfil=\cdot\mid X}$
    such that
        $\ffil(0|0) \geq \ffil(0|1)$.
%   Denote $\ffil(0|0) = \pi_0$ and $\ffil(0|1)=\pi_1$.

\item The filter chooses its \emph{action} $\afil\in\bin$: whether to block the content ($\afil=0$) or to forward it to the consumer ($\afil=1$). If the filter blocks, the game ends. Else, the game continues as follows.

\item The consumer chooses how much effort to put into examining the content. Formally, the consumer chooses a conditional distribution $\fcon\rbr{\cdot\mid X}$ over $\bin$, a.k.a. \emph{information strategy}.

\item The consumer examines the content. Formally, the consumer receives a signal $\scon\in\bin$ about the content type, drawn independently from
        $\fcon\rbr{\cdot\mid X}= \Pr\sbr{\scon=\cdot\mid X}$.
    Here, $\scon=0$ means ``likely malicious" and $\scon=1$ means ``likely legitimate".

\item The consumer chooses its \emph{action} $\acon\in\bin$: whether to accept the content as legitimate ($\acon=1$) or to ignore it ($\acon=0$).

\end{enumerate}

\nicomment{I find this emphasis on pure strategies more distracting than useful; recommend just introducing mixed (and I don't see a point to making a distinction for $\fcon$). If you want to talk about pure strategies later, you can still use the mixed notation and simply note that the strategy in that case is pure.  Here's a recommendation for replacing this paragraph: ``The filter and consumer choose action strategies $\mixstrfil$ and $\mixstrcon$, respectively. These strategies are random mappings from the agent's signal to their action.  The consumer additionally selects an information strategy $\fcon$. We denote a generic mixed strategy profile by $\mixsigma$ and its component action strategies of the filter and consumer by $\mixstrfil$ and $\mixstrcon$, respectively.''}
The filter and the consumer choose their \emph{action strategies} $\strfil,\strcon:\bin\to\bin$ which determine their actions:
    $\afil = \strfil(\sfil)$ and $\acon = \strcon(\scon)$.%
\footnote{Abstractly, (pure) action strategies are mappings $\bin\to\bin$. A mixed action strategy is a distribution over them.}
Thus, pure strategies in the \ourGame are $\strfil$ for the filter, and $(\strcon,\fcon)$ for the consumer. Pure strategy profiles are represented as triples $\sigma = (\strfil,\strcon,\fcon)$. For a mixed strategy profile $\mixsigma$, let $\mixstrfil$ and $\mixstrcon$ be the mixed action strategies for the filter and consumer, respectively. 

\nicomment{I would create a new paragraph called {\bf Solution Concept.} and put it after the paragraphs on {\bf Utilities.}.}
We are interested in Perfect Bayesian Equilibria (PBE) in this game, with respect to utilities defined below.%
\footnote{Recall that in a PBE, the players choose their strategies to maximize their respective utilities under the usual constraints that beliefs are updated through Bayes rule.}
\nicomment{New paragraph: We analyze the perfect Bayesian equilibria (PBE) of our game.  A strategy profile $\mixsigma$ together with a belief $q_\con$ of the consumer about the content type $X$ is a PBE if: a) the consumer best-responds to the filter given belief $q_\con$, b) the consumers' beliefs are consistent with a Bayesian update given the filter's strategy and action, and c) the filter best-responds to the consumer.}

\nicomment{I would defer this to the section on the endogenous attacker; it's too much to hold in my head and isn't relevant for a long while...}
We also consider an extension with \emph{endogenous attacker}: a third strategic player called \emph{attacker} who chooses the distribution of $X$ before the \ourGame starts (see Section~\ref{sec:endog}).

For notation, the distribution of $X$ is characterized by $q = \Pr[X=0]$, the prior probability that the content is malicious. The distribution of filter's signal $\sfil$ is characterized by two numbers:
\begin{align}\label{eq:pi-defn}
    \pi_x = \Pr\sbr{\sfil=0\mid X=x} \qquad\text{for $x\in\bin$}.
\end{align}
(So, if the goal of $\sfil$ is to flag malicious messages ($X=0$), then
$\pi_0$ is the true positive rate and $\pi_1$ is the false positive rate.)
%    $\pi_x = \Pr\sbr{\sfil=0\mid X=x}$ for $x\in\bin$.
Likewise, the distribution of consumer's signal $\scon$ is characterized by
    $\mu=\rbr{\tilde{\pi}_0, \tilde{\pi}_1}$,
where
    $\tilde{\pi}_x=\Pr\sbr{\scon=0\mid X=x}$.
%, or equivalently a randomized mapping $\bin\to\bin$; by abuse of notation, we allow both interpretations.
\nicomment{seems like a lot of notation, do we really need it all? e.g., do we use $\mu$? and do we need both $\pi$ and $f(\cdot|\cdot)$?}
\ascomment{we may remove some of this notation once the body stabilizes ...}
\nicomment{good, then i'd also put $q,\pi$ in the itemized list explaining the timing of the game. it took me 2 or 3 skims to find the definition of $q$ the first time i was reading this.  if you do what i suggest, this entire paragraph will disappear.}

\xhdr{Utilities.}
The consumer's utility is the difference between the \emph{action payoff} $u(\afil\cdot\acon,X)$, determined by how the actions match the content type, and the \emph{information cost} for examining the content.

For action payoff, we interpret the product $\afil\cdot\acon\in\bin$ as an aggregate action: indeed, the content is consumed as legitimate if $\afil\cdot\acon=1$, and ignored otherwise. Thus, action payoffs are summarized by a $2\times 2$ table, see Table~\ref{tab:payoffs}. The consumer receives a reward when legitimate content is accepted ($\afil\cdot\acon=X=1$), and penalties if the content is missclassified ($\afil\cdot\acon\neq X$). We normalize action payoffs to $0$ if malicious content is ignored ($\afil\cdot\acon=X=0$).

\begin{table}[t]
\centering
\begin{tabular}{l|l|l}
   & $X=0$  & $X=1$  \\ \hline
$a_{\fil}\cdot a_{\con}=0$  & 0      & $-c_1$ \\ \hline
$a_{\fil} \cdot a_{\con}=1$ & $-c_2$ & $b$    \\
\end{tabular}
\caption{Action payoffs $u(\afil\cdot\acon,X)$: reward $b\geq 0$ and penalties $c_1,c_2\geq 0$.}
\label{tab:payoffs}
\end{table}

The information cost is interpreted as the cost for obtaining signal $\scon$ about content type $X$, which only happens in the event when $\afil=1$. More abstractly, we consider the information cost for obtaining some randomized signal $\signal$ about some hidden state $X$ given some event $\mE$, denoted
    $\infoC\sbr{\signal; X \mid \mE}$
and determined by the conditional joint distribution of $(\signal,X)$
given $\mE$. We adopt the definition from \cite{sims1}, which is
well-established in prior work \cite{martin,bertoli,ravid}.
%\asmargincomment{cite to substantiate?}
\begin{align}\label{eq:cost-defn}
 \infoC\sbr{\signal;X \mid \mE}
    = \infoL\cdot I\rbr{\signal;X \mid \mE},
\end{align}
where $I\rbr{\signal;X \mid \mE}\geq 0$ is the mutual information conditional on the event $\mE$ and $\infoL>0$ is a known parameter. Thus, the information cost incurred when the consumer examines the content is defined via \eqref{eq:cost-defn} as
    $\infoC\sbr{\scon;X \mid \afil=1}$.
Some of our results carry over to a general model of information costs which only makes concavity/convexity assumptions, see Section~\ref{sec:generalized-costs}.

To summarize: the consumer's expected utility for strategy profile $\sigma = (\strfil,\strcon,\fcon)$ is
\begin{align}
\Vcon(\sigma) = \E_{X,\sfil,\scon}\sbr{ u(\acon\cdot\afil,X) - \ind{\afil=1}\cdot\infoC\sbr{\scon;X \mid \afil=1}}.
\end{align}
As a shorthand, denote the expected action cost for a given $\sigma$ as
    $u(\sigma) = \E_{X,\sfil,\scon}\sbr{ u(\acon\cdot\afil,X)}$,
and the information cost as
    $\infoC(\sigma) = \infoC\sbr{\scon;X \mid \afil=1}$.
\nicomment{i might have preferred swapping $V$ and $u$ and saying the expected utility, now represented by $u$, is the value $V$ minus the cost. but probably not worth changing notation right now.}

\nicomment{this paragraph should be swapped with the one before it imo.}
Since
    $I(\signal;X) = H(X)-H(\signal|X)$,
the information cost \eqref{eq:cost-defn} is proportional to the reduction in consumer's uncertainty about $X$, where the uncertainty is expressed via entropy $H$. The information cost is $0$ if and only if the signal is \emph{uninformative}, in the sense that
    $\Pr\sbr{X=\cdot\mid \signal,\mE}$
does not depend on $\signal$. The information cost
    $\infoC\sbr{\scon;X \mid \afil=1}$
depends not only on the conditional distribution of $\scon$ chosen by the consumer, but also on the filter's action strategy $\strfil$, because $\strfil$ impacts the posterior distribution given $\afil=1$. \nicomment{might be helpful to calculate the expected utility, or at least cost, for some choice of filter accuracy/strategy and user attention}

We posit that filter's utility is largely aligned with the consumer's. We consider two variants:
\begin{description}

\item[Aligned utilities] The two utilities are exactly equal. The filter's objective is to serve the  consumer. This may reflect the incentives of a large commercial email provider or a social networking service.

\item[Semi-aligned utilities] The filter's utility includes the action payoff $u(\acon,\afil,X)$, but not the information cost. This may better reflect, \eg incentives of a large employer with respect to internal email traffic.
\end{description}
%In more general variants (not considered in this paper), the filter may experience different action payoffs, or share some information costs.
The filter's expected utility for strategy profile $\sigma = (\strfil,\strcon,\fcon)$ is denoted $\Vfil(\sigma)$. In our notation, $\Vfil(\sigma) = \Vcon(\sigma)$ for aligned utilities, and $\Vfil(\sigma)=u(\sigma)$ for semi-aligned utilities. For a \emph{mixed} strategy profile $\mixsigma$, we use the same notation:
    $V_i(\mixsigma) := \E_{\sigma\sim\mixsigma} V_i(\sigma)$ for $i\in\{\fil,\con\}$.

\xhdr{Model parameters.} Our model is specified by several parameters: \emph{payoff parameters} $b,c_1,c_2,\infoL$ which characterize action payoffs and information costs, and \emph{distribution parameters} $q$\niedit{ and $\pi_0,\pi_1$} which characterize the \niedit{distribution of $X$ and the} joint distribution of $(X,\sfil)$\niedit{, respectively}.

\xhdr{Marginal value of technology.}
We are particularly interested in the marginal value of improving the filter's technology, \ie the filter's signal $\sfil$. We represent the quality of $\sfil$ as a pair $(\pi_0,1-\pi_1)\in[0,1]^2$, as defined in \eqref{eq:pi-defn}, so that componentwise increases correspond to increasing quality.
% so that increasing $\pi_0$ or decreasing $\pi_1$ improves the quality of $\sfil$.
We analyze \emph{comparative statics}, changing $\pi_0,\pi_1$ while keeping the other parameters fixed. Concretely, we fix an objective $\Vopt = \Vopt(\pi_0,\pi_1)$. \eg socially optimal equilibrium payoffs for aligned utilities, and interpret it as the \emph{value of technology} (VoT). Then, the marginal VoT is the pair
    $\rbr{\frac{\partial \Vopt}{\partial \pi_0},\, -\frac{\partial \Vopt}{\partial \pi_1} }$.
We say marginal VoT is positive if both components are positive, so that improving the quality of $\sfil$ improves the objective. Our main results establish a trichotomy between constant, linear, and non-linear VoT  as a function of $(\pi_0,\pi_1)$. \nicomment{don't understand the last sentence, isn't VoT a function of all model parameters, are we saying the form of the partial derivative doesn't depend on payoff/distribution parameters other than $\pi$? After talking to Alex, I think you mean something like: ``We show there are three regimes that describe the functional form of the dependence of the marginal VoT on the filter quality: constant, linear and non-linear. In a non-strategic environment, i.e., one with a naive filter that forwards all content that passes the classifier and a naive consumer who blindly accepts content forwarded by the filter, a marginal improvement in filter quality has a proportional improvement in the outcome.  Hence the marginal VoT is linear in filter quality.  If the cost of consuming malicious content is high and the filter is far from perfect, strategic agents will block/ignore all content.  Hence the marginal VoT is constant in filter quality. Interestingly, the strategic game induces a non-linear region as well.  In the following section, we derive bounds on beliefs that will help us delineate these three regions.''}

%Specifically, we consider an equilibrium strategy profile
%    $\sigma^* = \sigma^*(\pi_0,\pi_1)$
%as a function of $(\pi_0,\pi_1)$, keeping all other parameters fixed. Thus, utilities
%    $\Vfil(\sigma^*)$ and $\Vcon(\sigma^*)$
%are now functions of $(\pi_0,\pi_1)$, too. We characterize their marginal change w.r.t. $\pi_0,\pi_1$, via
%partial derivatives and/or discrete jumps.

\xhdr{A taxonomy for strategy profiles.}
\nicomment{this really feels like it belongs in the next section}
A strategy profile is called \emph{consumer-optimal} if the consumer best-responds to the filter's strategy. \nicomment{doesn't the consumer always best-respond given the filter moves first? i think we need to make our equil notion mathematically precise. Okay, I see now that you mean this is a subset of profiles and a superset of equilibria because you are leaving in some profiles where the filter does not best-respond.  How about replacing last sentence with: ``We will focus attention on a subset of strategy profiles that contain all PBE, namely those in which the consumer is best-responding to the filter given the belief (note this is a superset of PBE as we do not require the filter to best-respond to the consumer).''} There are only four possible action strategies, and therefore only four pure, consumer-optimal strategy profiles, see Table~\ref{tab:profiles}. The lower-left cell, where the filter reverses its signal ($\strfil(\psi)\neq \psi$), is unreasonable. \nicomment{i'd make table 2 be about the blocking/forwarding/diff strategy, not profile and then introduce that first and then introduce the profile stuff}
We name the other three:
%
the \emph{blocking profile} $\blkprof$
in which the filter always blocks the content: $\strfil(\cdot) \equiv 0$,
%
the \emph{forwarding profile} $\fwdprof$
in which filter always forwards the content: $\strfil(\cdot) \equiv 1$,
%
and the \emph{differentiating profile} $\difprof$
in which the filter differentiates between the signals: $\strfil(\psi) \equiv \psi$.
%
Similarly, the \emph{blocking strategy} $\strblk$ , the \emph{forwarding strategy} $\strfwd$, and the \emph{differentiating strategy} $\strdif$ is an action strategy $s:\bin\to\bin$ such that, resp., $s(\cdot) \equiv 0$, $s(\cdot) \equiv 1$, and $s(\psi) \equiv \psi$.
%
\asedit{We will prove that it suffices to consider $\difprof$ and $\fwdprof$, in the sense that one of them an equilibrium \emph{and} weakly Pareto-dominates any other mixed equilibrium (see Propositions~\ref{prop:aligned-best-eq} and ~\ref{prop:semi-eq}).}


%\begin{itemize}
%
%\item The \emph{differentiating profile} $\diffEqm$ is the consumer-optimal strategy profile  in which the filter's policy is \emph{differentiating}:
%    $\strfil(1) = 1$ and $\strfil(0) = 0$.
%%Thus, the filter does not strategically obfuscate its signal.
%
%\item The \emph{forwarding profile} $\fwdEqm$ is the consumer-optimal strategy profile in which the filter ignores its signal and always forwards the message: $\strfil\equiv 1$.
%
%\item The \emph{blocking profile} $\blkEqm$ is the consumer-optimal strategy profile in which the filter ignores its signal and always blocks the message: $\strfil\equiv 0$.
%\end{itemize}

\begin{table}[t]
\begin{center}
\begin{tabular}{r|l|l}
    & $\strfil(1)=0$
    & $\strfil(1)=1$
\hlinestrut
$\strfil(0)=0$
    & \emph{blocking profile} $\blkprof$
    & \emph{differentiating profile} $\difprof$
\hlinestrut
$\strfil(0)=1$
    & (unreasonable)
    & \emph{forwarding profile} $\fwdprof$
\end{tabular}
\end{center}
\caption{Consumer-optimal strategy profiles given the filter's action strategy $\strfil$.}
\label{tab:profiles}
\end{table}



==> prelim-Jan17.tex <==
%\section{Results with Exogenous Attacker}

The filter effectively has three pure strategy profiles: block all
content, forward all content and condition its action on its signal.
As will be shown, the value of information when the filter does not
condition its action on its signal is trivially $0$ since the filter's
signal does not impact its action.  Furthermore, if the consumer does
not incur information costs (i.e. either accepts all content or
ignores all content), the value of information is once again
trivial. To establish these results and gain insight into the more
interesting case in which the filter conditions its actions on its
signal and the consumer incurs positive information costs, we employ
the following definitions.

% Nevertheless, since these are the three main profiles that will
% characterize the equilibrium, we formally define them in definition
% \ref{def:first} for reference




% we do not rule out any possible equilibria, regardless of how
% trivial they may seem.  For example, we do not explicitly rule out
% equilibria where the filter's action does not depend on its signal,
% and thus it either passes all content to the consumer or blocks all
% content.  In this case, the marginal impact of improving the filter's
% signal is zero since it's action is independent of its signal.  From
% the consumer's perspective, we do not, ex-ante, rule out equilibria in
% which they incur no information costs and simply either accept or
% ignore all content.  In this case, the marginal impact of improving
% the filter's quality is also trivial, as we will show below.  However,
% one particular salient joint strategy profile is one in which the
% filter does indeed provide information to the consumer through its
% actions and the consumer incurs some attention cost to obtain further
% information.  It is in this case, \emph{and only this case}, where
% improving the filter's quality may have a non-trivial impact on
% outcomes.  We call this a \emph{differentiating equilibrium} and
% define it as follows:

\begin{defn}
  \label{def:first}
  \begin{enumerate}
    \item[]
  \item The \emph{filter-differentiating strategy},
      $\bar{s}_{\mathtt{f}}$, is the strategy given by
      $\bar{s}_{\mathtt{f}}(0)=0$ and $\bar{s}_{\mathtt{f}}(1)=1$.
    \item A \emph{consumer-differentiating action strategy},
      $\bar{s}_{\mathtt{c}}$ is an action strategy for the consumer where
      $\bar{s}_{\mathtt{c}}(0)=0$ and $\bar{s}_{\mathtt{c}}(1)=1$.
    \item A \emph{consumer-optimal, filter-differentiating}, joint strategy
    profile $\sigma^d$ is a joint strategy profile where the filter
    plays a filter-differentiating strategy and the consumer best
    responds (not necessarily with a consumer-differentiating
    strategy).
    \item A \emph{differentiating equilibrium},
      $\sigma^*=(s^*_{\mathtt{f}}, s^*_{\mathtt{c}}, \mu^*)$ is a
      perfect Bayesian equilibrium where
      $s^*_{\mathtt{f}}= \bar{s}_{\mathtt{f}}$ and
      $s^*_{\mathtt{c}}=\bar{s}_{\mathtt{c}}$.  with expected payoff
      $V_i(\sigma^*) = R(\sigma^*) - \lambda_i I(\sigma^*)$ for player
      $i$.
    \item A \emph{non-differentiating} profile, $\sigma^s$, is a joint
      strategy profile where the filter forwards all content and the
      consumer responds optimally.
    \item A \emph{blocking profile}, $\sigma^b$, is one in which the consumer
    blocks all content.
    \end{enumerate}
  \end{defn}

  We begin with proposition \ref{prop:regimes} that partitions the
  parameter space and derives consumer best responses in a subset of
  those parameter regimes.  These best responses in some regimes lead
  to rather trivial marginal value of information results, which we
  derive in corollary \ref{cor:regimes}.  Specifically, if the filter
  does not condition its message on its signal the marginal value of
  information is $0$.  Furthermore, if the consumer simply accepts all
  content the filter forwards, then the marginal value of information
  is just a linear function of the payoffs.

%   region in parameter space where the equilibrium and the value of
%   improving the filter's quality is trivial.  This allows us to focus
%   our subsequent analysis on the non-trivial differentiating
%   equilibrium.  The characterization of the non-differentiating
%   equilibria is given in proposition \ref{prop:regimes}.

\begin{prop}\label{prop:regimes}
  Let $\tilde{q} = \frac{(1-\pi_0)q}{(1-\pi_0)q + (1-\pi_1)(1-q)} =
  P(X=1|s_{\mathtt{f}} = \bar{s}_{\mathtt{f}}, a_{\mathtt{f}}=1)$,
  which is probability that the content is malicious conditional on
  the filter not blocking under strategy $\bar{s}_{\mathtt{f}}$.
  Then there exists values $q_H$ and $q_L$ with $q_H>q_L$ such that
  % $q_H= \frac{e^{b/\lambda}
  %   -e^{-c_1/\lambda}}{e^{b/\lambda}-e^{-(c_1+c_2)/\lambda}}$ and
  % $q_L=e^{-c_2/\lambda}q_H$.  Then:
  \begin{enumerate}
  \item if $\tilde{q}>q_H$ % ($q>q_H$),
    the consumer's dominant strategy is to ignore  all content.
    %and thus always ignoring is a best response to
      % $\bar{s}_{\mathtt{f}}$ (a filter that never blocks)
    \item If $\tilde{q}<q_L$, then accepting all content is the consumer's best
      response to $\bar{s}_{\mathtt{f}}$
    \item If $q<q_L$, then accepting all content is the consumer's
      dominant strategy.
    \end{enumerate}
  \end{prop}




  \begin{cor}\label{cor:regimes}
  For $i\in\{\texttt{f}, \texttt{c}\}$,
  \begin{enumerate}
      \item $\frac{\partial V_i(\sigma^d)}{\partial
      \pi_0}=\frac{\partial V(\sigma^d)}{\partial \pi_1} = 0$ if
    $\tilde{q}>q_H$
    \item $\frac{\partial V_i(\sigma^d)}{\partial
      \pi_0} = c_2>0$ and $\frac{\partial V(\sigma^d)}{\partial
      \pi_1} = -(c_1+b)<0$ if $\tilde{q}<q_L$
    \item $\frac{\partial V(\sigma^{\prime})}{\partial \pi_0} =
      \frac{\partial V_i(\sigma^{\prime})}{\partial \pi_1}=0$ for any
      $\sigma^{\prime}$ where the filter either blocks all content or
      forwards all content and the consumer responds optimally.
    \end{enumerate}
\end{cor}

In addition to providing consumer best responses, proposition
\ref{prop:regimes} highlights that importance of the consumer's belief
that content is malicious prior to incurring any information costs.
When the consumer's belief is outside of $[q_L, q_H]$ the consumer is
sufficiently sure of the content's legitimacy that it is not
worthwhile to further deliberate to gain a stronger signal.  Corollary
\ref{cor:regimes} then states the trivial result that if the consumer
does indeed block all content, there is no benefit to increasing the
filter's quality \emph{or} if the consumer simply accepts all content,
the value of information is as if the consumer were naive and
non-strategic.  Furthermore, if the filter does not condition its
actions on the signal it receives, then changing the quality of the
signal trivially has no impact on payoffs.  The results are summarized
in table \ref{tab:regimes}.




\begin{table}[h]

\begin{tabular}{ll|llll|}

\cline{3-6}

                                                         &                                          & \multicolumn{4}{c|}{Parameter Regime}                                                                                                                                                                                                                        \\ \hhline{~|-|-|-|-|-|} \hhline{~|-|-|-|-|-|}

\multicolumn{1}{l|}{}                                    &      \cellcolor[HTML]{EFEFEF}                                    & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}$\tilde{q}<q<q_L<q_H$} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}$\tilde{q}<q_L<q<q_H$} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}$q_L<\tilde{q}<q<q_H$} & \cellcolor[HTML]{EFEFEF}$q_L<\tilde{q}<q_H<q$ \\ \hline

\multicolumn{1}{|c|}{}                                   & \cellcolor[HTML]{EFEFEF}$\sigma^d$ & \multicolumn{1}{l|}{ \cellcolor[HTML]{CCFFC7}$c_2,  -(c_1 + b)$}                            & \multicolumn{1}{l|}{\cellcolor[HTML]{CCFFC7} $c_2, -(c_1+b)$}                               & \multicolumn{1}{l|}{?}                                             & ?                                             \\ \hhline{~|-|-|-|-|-|}

\multicolumn{1}{|c|}{\multirow{-2}{*}{Strategy Profile}} & \cellcolor[HTML]{EFEFEF}$\sigma^s$       & \multicolumn{1}{l|}{\cellcolor[HTML]{CCFFC7}$0,0$}                                         & \multicolumn{1}{l|}{0,0}                                             & \multicolumn{1}{l|}{\cellcolor[HTML]{FF8383}$0,0$}                                         & \cellcolor[HTML]{FF8383} $0,0$                                         \\ \hline

\end{tabular}
\caption{Marginal value of information and consumer best response for
  different filter, strategy profiles     The first term in each cell is
  $\frac{\partial V_i(\sigma)}{\partial \pi_0}$ while the second term is
  $\frac{\partial V_i(\sigma)}{\partial \pi_1}$ for $i \in \{textt{f},
  \texttt{c}\}$. The green cells are
  where the consumer's best response is to accept all content, the red
cells are where the consumer's best response is to ignore all
content.  The marginal value of information is always $0$ under
$\sigma^b$ and when $\tilde{q}>q^H$, which is omitted from the table.}
\label{tab:regimes}
\end{table}


Of course, the ultimate goal is to determine the value of information
in \emph{equilibrium}.  What then remains to be shown the value of
information at the remaining strategy profiles not shown in table
\ref{tab:regimes} and characterize when each profile is the (socially
optimal) equilibrium.  For completeness, the following proposition
shows that any mixed strategy equilibrium is dominated by $\sigma^b$
and allows us to focus on pure strategy equilibria.

\begin{prop}\label{prop:nomix}
  There does not exist a mixed strategy equilibrium with payoffs
  greater than $V(\sigma^b)$..
\end{prop}



% Proposition \ref{prop:regimes} says that a differentiating equilibrium
% can \emph{only} exist if $q_L<\tilde{q}<q_H$ since outside that
% region, the consumer's optimal strategy is not to differentiate.  When
% $\tilde{q}>q_H$, then the consumer has such high certainty that the
% content is malicious that it is not worthwhile to invest attention
% resources to determining the legitimacy of the content and simply
% blocks all content.  On the other hand, when $\tilde{q}<q_L$, the
% consumer is sufficiently certain that the content is legitimate that
% it accepts the content without inspection.

% When $\tilde{q}$ lies outside of $[q_L, q_H]$ the
% consumer's strategy is fixed and it does not incur information costs.
% In these regimes it is straightforward to quantify the impact of
% marginal changes in the filter's quality when the filter plays a
% differentiating strategy.  We do this by examining independent
% marginal changes in $\pi_0$, the filter's true positive rate, and
% $\pi_1$ the filter's false positive rate.  Those derivatives are given
% in corollary \ref{cor:regimes}.


% Furthermore, corollary \ref{cor:regimes} establishes that under a
% differentiating profile, when $\tilde{q}>q_H$ small changes to the
% filter quality are trivially zero since the consumer is going to block
% all content anyway.  When $\tilde{q}<q_L$ the marginal value of the
% filter quality is the same as if the consumer was non-strategic and
% simply accepted all content.


% \begin{defn}
%   \label{def:oprof}
%   \begin{itemize}
%   \item[]
%   \item A \emph{non-differentiating} profile, $\sigma^s$, is a joint strategy
%   profile where the filter forwards all content and the consumer responds
%   optimally.
%   \item A \emph{filter-deceiving} strategy profile, $\sigma^t$, is a joint
%     strategy profile where the filter forwards all content but the
%     consumer responds optimally, \emph{as if} the filter played a
%     differentiating strategy.
%   \item A \emph{blocking profile}, $\sigma^b$, is one in which the consumer
%     blocks all content
%   \end{itemize}
% \end{defn}



